Visualizing information on watch faces: A survey with smartwatch users

People increasingly wear smartwatches that can track a wide variety of data. However, it is currently unknown which data people consume and how it is visualized. To better ground research on smartwatch visualization, it is important to understand the current use of these representation types on smartwatches, and to identify missed visualization opportunities. We present the findings of a survey with 237 smartwatch wearers, and assess the types of data and representations commonly displayed on watch faces. We found a predominant display of health & fitness data, with icons accompanied by text being the most frequent representation type. Combining these results with a further analysis of online searches of watch faces and the data tracked on smartwatches that are not commonly visualized, we discuss opportunities for visualization research.

==> sections/06-conclusion.tex <==



\section{Conclusion} 
%One of our initial goals for our survey and online search of smart-watch faces was to provide answers to ground or more easily target future research on smartwatch visualizations.
We conducted a survey on smartwatch use and an online search of smartwatch faces, in order to to ground or more easily target future research on smartwatch visualizations.
%We saw that participants most frequently saw data from the health/fitness category on their watch faces. When designing future perceptual studies and tasks, taking participants' familiarity with step counts, temperature measurements, or battery level into account might be useful for quantitative data. The most common categorical data participants saw on their watch faces was weather information (sun vs.\ rain). 
%
%We saw that people had a relatively high number of data items on their watch faces (5 on average). This number of 5 different amounts of data on average can help to design new watch faces that show data with visualizations that people care about the most. Yet, an open question for research is how people can actually cope with such a dense data display, in particular if participants chose to show 5 different colorful visualizations on their watch faces. 
In our paper we highlight commonly tracked and commonly seen data, how many are present on watch faces at any given time, and how these are represented. Based on these findings, we highlight the still limited use of visualizations, identify opportunities for visualizing commonly tracked (but under-represented) data, and discuss possible research directions in smartwatch visualization research.   

%Some of our findings also open new questions. For example it is unclear if the choices of data representations is a personal preference or a choice enforced by watch face designers. 


==> sections/authors-anonymous.tex <==
\author{author names removed for blind review}




==> sections/copyright.tex <==
%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
\setcopyright{acmcopyright}
\copyrightyear{2018}
\acmYear{2018}
\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
\acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural
  Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
\acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
  June 03--05, 2018, Woodstock, NY}
\acmPrice{15.00}
\acmISBN{978-1-4503-XXXX-X/18/06}


%%
%% Submission ID.
%% Use this when submitting an article to a sponsored event. You'll
%% receive a unique submission ID from the organizers
%% of the event, and this ID should be used as the parameter to this command.
%%\acmSubmissionID{123-A56-BU3}

%%
%% The majority of ACM publications use numbered citations and
%% references.  The command \citestyle{authoryear} switches to the
%% "author year" style.
%%
%% If you are preparing content for an event
%% sponsored by ACM SIGGRAPH, you must use the "author year" style of
%% citations and references.
%% Uncommenting
%% the next command will enable that style.
%%\citestyle{acmauthoryear}

%%
%% end of the preamble, start of the body of the document source.

==> sections/keywords.tex <==
%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
\keywords{datasets, neural networks, gaze detection, text tagging}
